Search for new phenomena in different-flavour high-mass dilepton final states in $pp$ collisions at $\sqrt{s}=13$ TeV with the ATLAS detector

A search is performed for a heavy particle decaying into different flavour dilepton pairs ($e\mu$, $e\tau$ or $\mu\tau$), using 3.2 $fb^{-1}$ of proton-proton collision data at $\sqrt{s}=13$ TeV collected in 2015 by the ATLAS detector at the Large Hadron Collider. No excess over the Standard Model prediction is observed. Limits at the 95% credibility level are set on the mass of a $Z^{\prime}$ boson with lepton-flavour-violating couplings at 3.0, 2.7 and 2.6 TeV, and on the mass of a supersymmetric $\tau$ sneutrino with $R$-parity-violating couplings at 2.3, 2.2 and 1.9 TeV, for $e\mu$, $e\tau$ and $\mu\tau$ final states, respectively. The results are also interpreted as limits on the threshold mass for quantum black hole production.

==> Sections/AnalysisStrategy.tex <==
The aim of this search is to find an excess in the $m_{e\mu}$ spectrum from
expectation that could point to Lepton-flavour violating decays, forbidden in
the Standard model (SM). 
For that purpose, electron-muon pairs are selected and their invariant mass is
calculated. The expected yields and $m_{e\mu}$ spectrum shape for the various SM
backgrounds is obtained through a combination of Monte Carlo simulation for the
physics backgrounds and a data-driven method for the instrumental ones. The
results obtained are compared to the observed $m_{e\mu}$ spectrum.
In the search phase, the aim is to test the background-only hypothesis through
the use of a frequentist LLR test to look for possible deviations from SM
expectation. If no globally significant deviations beyond $3\sigma$ are found,
exclusion limits for the parameter of interest of the various models searched
are extracted. A Bayesian method is used to find the 95\% CL exclusion limits 
on the parameter of interestest of these new physics models ($m_{\Zprime}$ and
$M_{\mathrm{th}}$).



==> Sections/auxiliary.tex <==
A full list of the choice of parameters used to generate the quantum black hole
samples with QBH 3.00 follows for the ADD (RS) model: 
\begin{itemize}
\item Beam 1 Energy = \SI{6.5}{\TeV};
\item Beam 2 Energy = \SI{6.5}{\TeV};
\item Extradimensional Planck Mass = minimum black hole mass, also known as
  $M_{\mathrm{th}}$, with $M_{\mathrm{th}}=x_{\mathrm{min}}*M_{\mathrm{D}}$. The
  variable $x_{\mathrm{min}}$ is the ratio between the threshold for black hole
  formation and the extradimensional Planck mass, and is taken to be one;
\item Maximum quantum black hole mass = 3$\cdot$extra-dimensional Planck mass;
\item Extra dimension model: ADD (Randall-Sundrum);
\item Total number of dimensions = 10 (5);
\item PDF = CTEQ6L1;
\item QCD scale of the PDF is the inverse of the gravitational radius;
\item Using PDG definition of the Planck Scale. For such a definition the
  function $k(n)$ for the ADD model takes the form:
  \begin{equation}
    \label{eq:PlanckScale}
    k(n) = \displaystyle \left( 2^{n}\sqrt{\pi}^{n-3}
    \frac{\Gamma(\frac{n+3}{2})}{n+2}  \right)^{\frac{1}{n+1}}\;,
  \end{equation}
  where $\Gamma(n) = \int^{\infty}_0 x^{n-1}e^{-x}dx$\;;
\item Yoshino-Rychkov factors for cross-section enhancement not used;
  %\cite{bib:YoshinoFactors}
  %Probably that will require some explanation
\item Two-particle decay probability not included. There exists the possibility
  of decays to more than two particles as explained in Section 4 of
  \cite{bib:Gingrich2009}, with the multiplicity probabilities shown in Table
  4. By considering this possibility, the branching ratio could be weighted by
  a factor accounting for the probability of a two particle decay;
\item Include a Standard Model Higgs particle with a mass of \SI{125}{\GeV};
\item Include graviton;
\item Assume neutrinos are only left-handed and considered to be Dirac fermions.
\end{itemize}

\begin{figure}[htb]
  \centering
  \subfloat[\Zprime cross-section times branching ratio]{
    \includegraphics[width=0.49\textwidth]{aux/Zprime_Xsec}
    \label{fig:Zprime_XsecXBR}
  }
  \subfloat[QBH cross-section times branching ratio]{
    \includegraphics[width=0.49\textwidth]{aux/QBH_Xsec}
    \label{fig:QBH_XsecXBR}
  }\\
  \subfloat[RPV $\tilde{\nu}_{\tau}$ cross-section times branching ratio]{
    \includegraphics[width=0.49\textwidth]{aux/SVT_Xsec}
    \label{fig:SVT_XsecXBR}
  }
  \caption{Monte Carlo generator cross-section times branching ratio for
    (a) \Zprime$\to \ell\ell^{\prime}$ versus \Zprime polemass, (b) for the two
    non-thermal black hole models against threshold mass, and (c) for $\tau$
    sneutrino ($\tilde{\nu}_{\tau}\to \ell\ell^{\prime})$ against
    $\tilde{\nu}_{\tau}$ polemass. The line shows an interpolation between the
    points.}
  \label{fig:SignalModels_XsecXBR}
\end{figure}

\begin{figure}[htb]
  \centering
  \subfloat[\Zprime$\to e\mu$]{
    \includegraphics[width=0.49\textwidth]{aux/Zprime_shapes_emu}
    \label{fig:Zprime_shapes_emu}
  }
  \subfloat[QBH$\to e\mu$]{
    \includegraphics[width=0.49\textwidth]{aux/QBH_shapes_emu}
    \label{fig:QBH_shapes_emu}
  }\\
  \subfloat[RPV $\tilde{\nu}_{\tau}\to e\mu$]{
    \includegraphics[width=0.49\textwidth]{aux/SVT_shapes_emu}
    \label{fig:SVT_shapes_emu}
  }
  \caption{Electron-muon invariant mass distributions for signal models:
    (a) \Zprime, (b) quantum black hole RS and (c) $\tau$ sneutrino
    ($\tilde{\nu}_{\tau}$).}
  \label{fig:SignalShapes_emu}
\end{figure}

\begin{figure}[htb]
  \centering
  \subfloat[\Zprime$\to e\tau$]{
    \includegraphics[width=0.49\textwidth]{aux/Zprime_shapes_etau}
    \label{fig:Zprime_shapes_etau}
  }
  \subfloat[QBH$\to e\tau$]{
    \includegraphics[width=0.49\textwidth]{aux/QBH_shapes_etau}
    \label{fig:QBH_shapes_etau}
  }\\
  \subfloat[RPV $\tilde{\nu}_{\tau}\to e\tau$]{
    \includegraphics[width=0.49\textwidth]{aux/SVT_shapes_etau}
    \label{fig:SVT_shapes_etau}
  }
  \caption{Electron-tau invariant mass distributions for signal models:
    (a) \Zprime, (b) quantum black hole RS and (c) $\tau$ sneutrino
    ($\tilde{\nu}_{\tau}$).}
  \label{fig:SignalShapes_etau}
\end{figure}

\begin{figure}[htb]
  \centering
  \subfloat[\Zprime$\to \mu\tau$]{
    \includegraphics[width=0.49\textwidth]{aux/Zprime_shapes_mutau}
    \label{fig:Zprime_shapes_mutau}
  }
  \subfloat[QBH$\to \mu\tau$]{
    \includegraphics[width=0.49\textwidth]{aux/QBH_shapes_mutau}
    \label{fig:QBH_shapes_mutau}
  }\\
  \subfloat[RPV $\tilde{\nu}_{\tau}\to \mu\tau$]{
    \includegraphics[width=0.49\textwidth]{aux/SVT_shapes_mutau}
    \label{fig:SVT_shapes_mutau}
  }
  \caption{Muon-tau invariant mass distributions for signal models:
    (a) \Zprime, (b) quantum black hole RS and (c) $\tau$ sneutrino
    ($\tilde{\nu}_{\tau}$).}
  \label{fig:SignalShapes_mutau}
\end{figure}

\begin{figure}[htb]
  \centering
  \subfloat[$e\mu$ channel]{
    \includegraphics[width=0.49\textwidth]{aux/Ae_emu}
    \label{fig:Ae_emu}
  }
  \subfloat[$e\tau$ channel]{
    \includegraphics[width=0.49\textwidth]{aux/Ae_etau}
    \label{fig:Ae_etau}
  }\\
  \subfloat[$\mu\tau$ channel]{
    \includegraphics[width=0.49\textwidth]{aux/Ae_mutau}
    \label{fig:Ae_mutau}
  }
  \caption{Acceptance times efficiency for the \Zprime model with
    lepton-flavour-violating coupling, supersymmetric $\tau$ sneutrino with
    $R$-parity-violating coupling (RPV SUSY $\tilde{\nu}_{\tau}$) and the
    quantum black hole (QBH) RS model for the (a) $e\mu$ , (b) $e\tau$  and
    (c) $\mu\tau$  channels.}
  \label{fig:Models_Ae}
\end{figure}

\begin{figure}[htb]
  \centering
  \subfloat[Top Quark fit variation: $e\mu$ channel]{
    \includegraphics[width=0.49\textwidth]{aux/FitVariation_emu}
  }
  \subfloat[Top Quark fit systematics: $e\mu$ channel]{
    \includegraphics[width=0.49\textwidth]{aux/FitSys_emu}
  }
  \caption{(a) The fit variation for the top quark background extrapolation in
    the $e\mu$ channel. The nominal fit and the variations are shown, together
    with the top quark background MC estimation. (b) The fit uncertainty band
    for the top quark background extrapolation in the $e\mu$ channel. It
    includes the full systematic uncertainty when adding the fit parameter
    uncertainty and the fit variation from the functions shown in equation~\ref{eq:djet-monimial} 
    in the paper. The points show the final estimation of the top quark background including MC and extrapolation.}
  \label{fig:extrapolationVariation_emu}
\end{figure}

\begin{figure}[htb]
  \centering
  \subfloat[Top Quark fit variation: $e\tau$ channel]{
    \includegraphics[width=0.49\textwidth]{aux/FitVariation_etau}
  }
  \subfloat[Top Quark fit systematics: $e\tau$ channel]{
    \includegraphics[width=0.49\textwidth]{aux/FitSys_etau}
  }
  \caption{(a) The fit variation for the top quark background extrapolation in
    the $e\tau$ channel. The nominal fit and the variations are shown, together
    with the top quark background MC estimation. (b) The fit uncertainty band
    for the top quark background extrapolation in the $e\tau$ channel. It
    includes the full systematic uncertainty when adding the fit parameter
    uncertainty and the fit variation from the functions shown in equation~\ref{eq:djet-monimial} 
    in the paper. The points show the final estimation of the top quark background
    including MC and extrapolation.}
  \label{fig:extrapolationVariation_etau}
\end{figure}

\begin{figure}[htb]
  \centering
  \subfloat[Top Quark fit variation: $\mu\tau$ channel]{
    \includegraphics[width=0.49\textwidth]{aux/FitVariation_mutau}
  }
  \subfloat[Top Quark fit systematics: $\mu\tau$ channel]{
    \includegraphics[width=0.49\textwidth]{aux/FitSys_mutau}
  }
  \caption{(a) The fit variation for the top quark background extrapolation in
    the $\mu\tau$ channel. The nominal fit and the variations are shown,
    together with the top quark background MC estimation. (b) The fit
    uncertainty band for the top quark background extrapolation in the
    $\mu\tau$ channel. It includes the full systematic uncertainty when adding
    the fit parameter uncertainty and the fit variation from the functions 
    shown in equation~\ref{eq:djet-monimial} in the paper. The points show the final estimation of the
    top quark background including MC and extrapolation.}
  \label{fig:extrapolationVariation_mutau}
\end{figure}


Tables \ref{tab:emu_yields}, \ref{tab:etau_yields} and \ref{tab:mutau_yields}
give a more detailed summary of the expected and observed yields in the
validation and search regions for each of the channels considered in this
search.
\begin{table}[htbp]
  \centering
  \footnotesize
  \subfloat[$N_{\mathrm{events}}$ with $m_{e\mu}<600$~\si{\GeV}]{
    \begin{tabular}{l|r@{\,}@{$\pm$}@{\,}l@{\,}|r@{\,}@{$\pm$}@{\,}l@{\,}}
      \hline\hline 
      Process          & \multicolumn{2}{c|}{$m_{e\mu}<300$~\si{\GeV}}
      & \multicolumn{2}{c}{$300<m_{e\mu}<600$~\si{\GeV}}\\
      \hline
      Top quark        &  \;\;\;\;\;840   & 90
                       &  \;\;\;\;\;\;\;\;\;\;350   & 40  \\
      Diboson          &  114   & 11
                       &   45   & 5   \\
      QCD and \W+jets  &   41   & 9
                       &   15   & 4   \\
      \DY              &   10.9 & 1.5
                       &    3.6 & 0.9 \\
      \hline
      Total background & 1010   & 100
                       &  410   & 50  \\
      \hline
      Data             & \multicolumn{2}{c|}{1040}
                       & \multicolumn{2}{c}{423}   \\
      \hline \hline
    \end{tabular}
  }\\
  \subfloat[$N_{\mathrm{events}}$ with $m_{e\mu}>600$~\si{\GeV}]{
    \begin{tabular}{l|r@{\,}@{$\pm$}@{\,}l@{\,}|r@{\,}@{$\pm$}@{\,}l@{\,}}
      \hline\hline 
      Process & \multicolumn{2}{c|}{$600<m_{e\mu}<1200$~\si{\GeV}}
      & \multicolumn{2}{c}{$1200<m_{e\mu}<2000$~\si{\GeV}} \\
      \hline
      Top quark        & \;\;\;\;\;\;\;\;\;\;\;\;\;21    & 6
                       & \;\;\;\;\;\;\;\;\;\;\;0.31 & 0.24  \\
      Diboson          & 4.8  & 0.9
                       & 0.16 & 0.11  \\
      QCD and \W+jets  & 2.7  & 1.7
                       & \multicolumn{2}{c}{-} \\
      \DY              & (1.7  & 0.3) $\cdot$ 10$^{-1}$ 
                       & (5    & 4  ) $\cdot$ 10$^{-3}$ \\
      \hline
      Total background & 29    & 7
                       &  0.47 & 0.34 \\
      \hline
      Data             &  \multicolumn{2}{c|}{24}
                       &  \multicolumn{2}{c}{0}  \\
      \hline \hline
      \multicolumn{5}{c}{}\\
      \hline \hline
      Process & \multicolumn{2}{c|}{$2000<m_{e\mu}<3000$~\si{\GeV}}
      & \multicolumn{2}{c}{$m_{e\mu}>3000$~\si{\GeV}}\\
      \hline
      Top quark        &  (0.8 & 1.8 ) $\cdot$ 10$^{-2}$
                       &  (1   & 5   ) $\cdot$ 10$^{-4}$  \\
      Diboson          &  (1.0 & 1.3 ) $\cdot$ 10$^{-2}$
                       &  (3   & 7   ) $\cdot$ 10$^{-4}$  \\
      QCD and \W+jets  &  \multicolumn{2}{c|}{-} 
                       &  \multicolumn{2}{c}{-}          \\
      \DY              &  (4   & 5   ) $\cdot$ 10$^{-4}$
                       &  (2   & 4   ) $\cdot$ 10$^{-5}$  \\
      \hline
      Total background &  (1.8 & 2.3 ) $\cdot$ 10$^{-2}$
                       &  (4   & 9   ) $\cdot$ 10$^{-4}$  \\
      \hline
      Data             &  \multicolumn{2}{c|}{1}
                       &  \multicolumn{2}{c}{0}          \\
      \hline \hline    
    \end{tabular}
  }
  \caption{Number of expected and observed $e\mu$ events in the validation (a)
    and search (b) regions. The quoted errors include statistical and
    systematic uncertainties.}
  \label{tab:emu_yields}
\end{table}

\begin{table}[htbp]
  \centering
  \footnotesize
  \subfloat[$N_{\mathrm{events}}$ with $m_{e\tau}<600$~\si{\GeV}]{
    \begin{tabular}{l|r@{\,}@{$\pm$}@{\,}l@{\,}|r@{\,}@{$\pm$}@{\,}l@{\,}}
      \hline\hline 
      Process          & \multicolumn{2}{c|}{$m_{e\tau}<300$~\si{\GeV}}
      & \multicolumn{2}{c}{$300<m_{e\tau}<600$~\si{\GeV}}\\
      \hline
      Top              &  \;\;\;\;\;480 &  110
                       &  \;\;\;\;\;\;\;\;\;\;310 &   80 \\
      Diboson          &   71 &   17
                       &   38 &    9 \\
      QCD and \W+jets  & 2700 &  700
                       &  510 &  140 \\
      \DY              &  890 &  200
                       &  133 &   32 \\
      \hline
      Total background & 4200 & 1000
                       &  990 & 250  \\
      \hline
      Data             & \multicolumn{2}{c|}{4424}
                       &  \multicolumn{2}{c}{992} \\
      \hline \hline               
    \end{tabular}
  }\\
  \subfloat[$N_{\mathrm{events}}$ with $m_{e\tau}>600$~\si{\GeV}]{
    \begin{tabular}{l|r@{\,}@{$\pm$}@{\,}l@{\,}|r@{\,}@{$\pm$}@{\,}l@{\,}}
      \hline\hline 
      Process & \multicolumn{2}{c|}{$600<m_{e\tau}<1200$~\si{\GeV}}
      & \multicolumn{2}{c}{$1200<m_{e\tau}<2000$~\si{\GeV}} \\
      \hline
      Top              & \;\;\;\;\;\;\;\;\;\;\;\;\;24    &  8 
                       & \;\;\;\;\;\;\;\;\;\;\;0.28 &  0.22 \\
      Diboson          & 5.7  &  1.7
                       & 0.48 &  0.28 \\
      QCD and \W+jets  & 44    & 14
                       &  1.2  &  0.6 \\
      \DY              &  5.0  &  1.3
                       & (2.0  &  1.1) $\cdot$ 10$^{-1}$ \\
      \hline
      Total background & 79    & 24
                       &  2.1  &  1.2 \\
      \hline
      Data             &  \multicolumn{2}{c|}{106}
                       &  \multicolumn{2}{c}{5}    \\
      \hline \hline
      \multicolumn{5}{c}{}\\
      \hline \hline
      Process & \multicolumn{2}{c|}{$2000<m_{e\tau}<3000$~\si{\GeV}}
      & \multicolumn{2}{c}{$m_{e\tau}>3000$~\si{\GeV}}\\
      \hline
      Top              &  (0.5 & 0.7) $\cdot$ 10$^{-2}$
                       &  (0.3 & 1.1) $\cdot$ 10$^{-4}$  \\
      Diboson          &  (3.2 & 2.9) $\cdot$ 10$^{-2}$
                       &  (1.7 & 2.3) $\cdot$ 10$^{-4}$  \\
      QCD and \W+jets  &  (6   & 4  ) $\cdot$ 10$^{-2}$
                       &  (4   & 6  ) $\cdot$ 10$^{-4}$  \\
      \DY              &  (1.5 & 0.9) $\cdot$ 10$^{-2}$
                       &  (5   & 7  ) $\cdot$ 10$^{-4}$  \\
      \hline                               
      Total background & (11   & 7  ) $\cdot$ 10$^{-2}$
                       & ( 1.1 & 1.5) $\cdot$ 10$^{-3}$  \\
      \hline
      Data             &  \multicolumn{2}{c|}{0}
                       &  \multicolumn{2}{c}{0}         \\
      \hline \hline    
    \end{tabular}
  }
  \caption{Number of expected and observed $e\tau$ events in the validation (a)
    and search (b) regions. The quoted errors include statistical and
    systematic uncertainties.}
  \label{tab:etau_yields}
\end{table}

\begin{table}[htbp]
  \centering
  \footnotesize
  \subfloat[$N_{\mathrm{events}}$ with $m_{\mu\tau}<600$~\si{\GeV}]{
    \begin{tabular}{l|r@{\,}@{$\pm$}@{\,}l@{\,}|r@{\,}@{$\pm$}@{\,}l@{\,}}
      \hline\hline 
      Process          & \multicolumn{2}{c|}{$m_{\mu\tau}<300$~\si{\GeV}}
      & \multicolumn{2}{c}{$300<m_{\mu\tau}<600$~\si{\GeV}}\\
      \hline
      Top              &  \;\;\;\;\;350 &   80
                       &  \;\;\;\;\;\;\;\;\;\;230 &   60 \\
      Diboson          &   56 &   13
                       &   29 &    7 \\
      QCD and \W+jets  & 1600 &  400
                       &  290 &   80 \\
      \DY              &  530 &  120
                       &   77 &   19 \\
      \hline
      Total background & 2600 &  600 
                       &  630 &  160 \\
      \hline
      Data             & \multicolumn{2}{c|}{2645}
                       & \multicolumn{2}{c}{594}   \\
      \hline \hline               
    \end{tabular}
  }\\
  \subfloat[$N_{\mathrm{events}}$ with $m_{\mu\tau}>600$~\si{\GeV}]{
    \begin{tabular}{l|r@{\,}@{$\pm$}@{\,}l@{\,}|r@{\,}@{$\pm$}@{\,}l@{\,}}
      \hline\hline 
      Process & \multicolumn{2}{c|}{$600<m_{\mu\tau}<1200$~\si{\GeV}}
      & \multicolumn{2}{c}{$1200<m_{\mu\tau}<2000$~\si{\GeV}} \\
      \hline
      Top              & \;\;\;\;\;\;\;\;\;\;\;\;\;21    & 7
                       & \;\;\;\;\;\;\;\;\;\;\; 0.4  & 0.5  \\
      Diboson          &  4.5  & 1.3
                       &  0.27 & 0.25 \\
      QCD and \W+jets  & 33    & 15
                       &  1.1  & 1.0  \\
      \DY              &  2.5  & 1.0
                       & 0.13  & 0.12 \\
      \hline
      Total background & 61    & 20
                       &  1.9  &  1.8 \\
      \hline
      Data             &  \multicolumn{2}{c|}{45}
                       &  \multicolumn{2}{c}{3}   \\
      \hline \hline
      \multicolumn{5}{c}{}\\
      \hline \hline
      Process & \multicolumn{2}{c|}{$2000<m_{\mu\tau}<3000$~\si{\GeV}}
      & \multicolumn{2}{c}{$m_{\mu\tau}>3000$~\si{\GeV}}\\
      \hline
      Top              &  (0.8 &  2.1) $\cdot$ 10$^{-2}$
                       &  (1   &  9  ) $\cdot$ 10$^{-4}$  \\
      Diboson          &  (2   &  4  ) $\cdot$ 10$^{-2}$
                       &  (7   & 10  ) $\cdot$ 10$^{-4}$  \\
      QCD and \W+jets  &  (4   &  7  ) $\cdot$ 10$^{-2}$
                       &  (1.6 &  1.8) $\cdot$ 10$^{-3}$  \\
      \DY              &  (1.3 &  1.9) $\cdot$ 10$^{-2}$
                       &  (1.4 &  2.1) $\cdot$ 10$^{-3}$  \\
      \hline
      Total background &  (0.9 & 1.4) $\cdot$ 10$^{-1}$
                       &  (4   & 5  ) $\cdot$ 10$^{-3}$   \\
      \hline
      Data             &  \multicolumn{2}{c|}{0}
                       &  \multicolumn{2}{c}{0}          \\
      \hline \hline    
    \end{tabular}
  }
  \caption{Number of expected and observed $\mu\tau$ events in the validation
    (a) and search (b) regions. The quoted errors include statistical and
    systematic uncertainties.}
  \label{tab:mutau_yields}
\end{table}

\begin{table}[!htbp]
  \centering
  \begin{tabular}{c|c|c|c|c|c|c}
    \hline \hline       
    Channel & $m_{\ell\ell^{\prime}}$ [\si{\GeV}]
    & $E_T^{\mathrm{miss}}$ [\si{\GeV}] & Lepton type & $p_{T_{\ell}}$ [\si{\GeV}]
    & $\eta_{\ell}$ & $\phi_{\ell}$ \\
    \hline\hline
    \multirow{2}{*}{$e\mu$} & \multirow{2}{*}{2089} &
    \multirow{2}{*}{72}  &
             $\mu^+$ & 617  & 0.29 & 0.4    \\
    & & &  $e^-$ & 1164 & 1.64 & -2.8  \\
    \hline
    \multirow{2}{*}{$e\tau$} & \multirow{2}{*}{1634} &
    \multirow{2}{*}{8.5}  &
               $e^-$ & 412 & -1.26 & 1.8 \\
    & & &  $\tau^+$ & 409 & 1.33  & -1.5 \\
    \hline
    \multirow{2}{*}{$\mu\tau$} & \multirow{2}{*}{1666} &
    \multirow{2}{*}{130.5}  &
              $\mu^+$ & 159 & 2.20  & 2.7 \\
    & & &   $\tau^-$ & 81  & -2.19 & -0.5 \\
    \hline\hline
  \end{tabular}
  \caption{Details on the highest-mass event selected in the $e\mu$, $e\tau$
    and $\mu\tau$ channels.}
  \label{tab:Evt_Details}
\end{table}

\begin{figure}[!hbtp]
  \centering
  \includegraphics[width=0.75\columnwidth]{aux/Event_emu}
  \caption{Event display for the highest-mass event for the $e\mu$ channel.
    The electron has a $p_{\mathrm{T}}$ of \SI{1164}{\GeV} and an $\eta$ of -2.8.
    The antimuon has an $p_{\mathrm{T}}$ of \SI{617}{\GeV} and an $\eta$ of 0.4.
    The missing transverse energy of the event is \SI{72}{\GeV}. The invariant
    mass of the electron-antimuon pair is 2089~\GeV.}
  \label{fig:VP1_emu}
\end{figure}
\begin{figure}[!hbtp]
  \centering
  \includegraphics[width=0.75\columnwidth]{aux/Event_etau}
  \caption{Event display for the highest-mass event for the $e\tau$ channel.
    The electron has a $p_{\mathrm{T}}$ of \SI{412}{\GeV} and an $\eta$ of -1.26.
    The antitau has an $p_{\mathrm{T}}$ of \SI{409}{\GeV} and an $\eta$ of 1.33.
    The missing transverse energy of the event is \SI{8.5}{\GeV}. The invariant
    mass of the electron-antitau pair is 1634~\GeV.}
  \label{fig:VP1_etau}
\end{figure}
\begin{figure}[!hbtp]
  \centering
  \includegraphics[width=0.75\columnwidth]{aux/Event_mutau}
  \caption{Event display for the highest-mass event for the $\mu\tau$ channel.
    The antimuon has a $p_{\mathrm{T}}$ of \SI{159}{\GeV} and an $\eta$ of 2.20.
    The tau has an $p_{\mathrm{T}}$ of \SI{81}{\GeV} and an $\eta$ of -2.19. The
    missing transverse energy of the event is \SI{130.5}{\GeV}. The invariant
    mass of the antimuon-tau pair is 1666~\GeV.}
  \label{fig:VP1_mutau}
\end{figure}

